Do Scaling Agile Frameworks Address Global Software Development Risks? An Empirical Study

Driven by the need to coordinate activities of multiple agile development teams cooperating to produce a large software product, software-intensive organizations are turning to scaling agile software development frameworks. Despite the growing adoption of various scalin g agile frameworks, there is little empirical evidence of how effective their practices are in mitigating risk, especially in global software develop ment (GSD), where project failure is a known problem. In this study, we develop a GSD Risk Catalog of 63 risks to assess the degree to which two scaling agile frameworks--Disciplined Agile Delivery (DAD) and the Scaled Agile Framework (SAFe)--address software project risks in GSD. We examined data from two longitudinal case studies implementing each framework to identify the extent to which the framework practices address GSD risks. Scaling agile frameworks appear to help companies eliminate or mitigate many traditional risks in GSD, especially relating to users and customers. How ever, several important risks were not eliminated or mitigated. These persistent risks in the main belonged to the Environment quadrant highlighting t he inherent risk in developing software across geographic boundaries. Perhaps these frameworks (and arguably any framework), would have difficulty all eviating, issues that appear to be outside the immediate control of the organization.

==> risks-observed-table.tex <==
% DO NOT EDIT
% This table is generated automatically; if you change it,
% your changes will be overwritten.
\midrule
\textbf{Quadrant 1: Customer Mandate} \tabularnewline
\midrule
\emph{Conflict between users} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{1}: ``Because they've [product managers] been in the US and I've been here.  There's also that product is so complex, the knowledge in the domain makes it has some barriers, having your peers respect your opinion on things.  Because no matter what, you're thinking, if you haven't had ideas or experience, it can be so much harder for them to hear your ideas.  with UX, there're so many guiding principles that are sort of failing universally, studying the users, making things simpler, don't bother them with a lot stuffs all the time.  That's sort of things that people could not appreciate and they wouldn't even hear it because they know the product, it works like this, and they assumed the customers wanted the way it was.''.}  \tabularnewline
\midrule
\emph{Lack of cooperation from users} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptOnePMO: ``I think the biggest challenge when it comes to the client and things we need to know from them and the follow up\ldots{} we need to do\ldots{} a little bit more internally you know.'') } \tabularnewline
\midrule
\emph{Lack of top management support for the project} (observed in Case B) \tabularnewline
\midrule
 {Case B: \Observation: Upper management occasionally overules decisions) } \tabularnewline
\midrule
\emph{Lack of user participation}  \tabularnewline
\midrule
\emph{Lack or loss of organizational commitment to the project}  \tabularnewline
\midrule
\emph{Users not committed to the project}  \tabularnewline
\midrule
\emph{Users resistant to change}  \tabularnewline
\midrule
\emph{Users with negative attitudes toward the project}  \tabularnewline
\midrule
\textbf{Quadrant 2: Scope and Requirements} \tabularnewline
\midrule
\emph{Conflicting system requirements} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{1}: ``The directions were, it's going to work on the iPad, make it as simple as possible\ldots{}  So, we did some great brainstorming sessions, there were a lot of fantastic ideas around that sort of thing, but then when we started on the project, stakeholder (the product management and POs) had different point of view, and it sort of switched from simplest possible to can you please translate what we have in the desktop app into the web.''.}  \tabularnewline
\midrule
 {Case B: \Observation: Large customer teams push for their fixes) } \tabularnewline
\midrule
\emph{Continually changing project scope/objectives} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptSevenSCAL: ``They [global customer] want a lot of stuff changed and then the main problem they have [is] localization.  Insurance is a big part in [the] [specific region] and it's very difficult there.  I think it's the most difficult and challenging part in our software.'') } \tabularnewline
\midrule
\emph{Continually changing system requirements} (observed in Case B) \tabularnewline
\midrule
 {Case B: } \tabularnewline
\midrule
\emph{Difficulty in defining the inputs and outputs of the system} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{1}: ``Before we had multiple features being built at the same time across the team, and the design work is done within the same time frame as the development, so it was very difficult to ask business to allocate the time to do design, we never got time to do research.  It was a bit of a rush.  We only had me and one other UX person, we might have 8 features, that's probably the worst, and it can be very complex.''.}  \tabularnewline
\midrule
\emph{Ill-defined project goals} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptNineSCAL: ``So, in that respect I find it difficult. We are kind of defining stuff as we go.  So, I haven't got strong reference point for why we are doing [the work on the project].'') } \tabularnewline
\midrule
\emph{Incorrect system requirements}  \tabularnewline
\midrule
\emph{System requirements not adequately identified} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{8}: ``No, we're not.  Here, there are aspects of a work here that is agile and aspects of our work that's not agile, and there's a large communication bottleneck.   Or non-collaborative thing\ldots{}   Probably what you would  the concept of product and release plan, although there have been significant changes recently we are not involved with it.''.}  \tabularnewline
\midrule
 {Case B: \transcriptThreeSCAL: ``\ldots{} the client would want to know a plan--they want to have a plan for everything that we [are] going to do.  Let's say, there are five change requests, for example, that's in-progress as in, we are still talking to them about what the requirement is.  So, there is no estimate on these.  They want to know exactly when they [are] all going to get done.'') } \tabularnewline
\midrule
\emph{Unclear system requirements} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptNineSCAL: ``So, in that respect I find it difficult. We are kind of defining stuff as we go.  So, I haven't got strong reference point for why we are doing [the work on the project].'') } \tabularnewline
\midrule
\emph{Undefined project success criteria} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptNineSCAL: ``So, in that respect I find it difficult. We are kind of defining stuff as we go.  So, I haven't got strong reference point for why we are doing [the work on the project].'') } \tabularnewline
\midrule
\emph{Users lack understanding of system capabilities and limitations}  \tabularnewline
\midrule
\textbf{Quadrant 3: Execution} \tabularnewline
\midrule
\emph{Development team unfamiliar with selected development tools} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{2}: ``We have a history of reinventing the wheel \ldots{} at what's out there that's going to make life easier for us to work, what problems already been solved.''.}  \tabularnewline
\midrule
\emph{Frequent conflicts among development team members} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptTwoSCAL: ``\ldots{} [W]e also had lot of conflicting sort of decisions within.  We had [porfolio role] who is the [team role], and a [Sr Developer] who is the Technical\ldots{} so that's been quite difficult as well.'') } \tabularnewline
\midrule
\emph{Frequent turnover within the project team}  \tabularnewline
\midrule
\emph{High level of technical complexity} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{2}: ``The thing that we have to deal with is that we have a lot of legacy code that was already built in those 3 tiers, and we brought a lot of that across \ldots{} we were sort of forced to stay with it because the need to reuse our code, we just didn't have time to build everything\ldots{} lot of room for improvement I think, if we started from scratch I think things will be a bit different.''.}  \tabularnewline
\midrule
 {Case B: \Observation: {[a given agile team role]} raises more issues than are solved) } \tabularnewline
\midrule
\emph{Highly complex task being automated} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{2}: ``[We] have about five sort of databases, each hosting a number of tenants, at least two different geographies, US and Europe.  I think our biggest database has got like 50 tenants in it, and the other are starting to fill up as well, and we've reached the limit before, and we just simply start up another server.  It is not a simple matter of one server, you have to, it's all clustered machines, you have to through 3-4 different servers you have to bring up to every new database.''.}  \tabularnewline
\midrule
\emph{Immature technology} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{2}: ``We're also not shy building our own tools, building our own code generators, things for specific problems, having ten people writing million lines of codes, which is also been our historical problems.''.}  \tabularnewline
\midrule
\emph{Inadequate estimation of project budget} (observed in Case B) \tabularnewline
\midrule
 {Case B: \Observation: Estimates vary widely from reality, usually too low) } \tabularnewline
\midrule
\emph{Inadequate estimation of project schedule} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptOneSCAL: ``We kind of overcommitted the first time. We overcommitted to a lot of stuff, work to be done within the sprint which I think was too much. It is a result of bad or wrong estimation. So, whatever we committed to do in two weeks in reality the job took four weeks.'') } \tabularnewline
\midrule
\emph{Inadequate estimation of required resources} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{4}: ``It's been years of reviewing, giving feedback, being overall it's going out, shortcut, running late, all over the walls with bugs, you know, you feel like you're trying to help, but there's no time for you.  So, that's been the bulk of the time, and now that the DAD process is coming I'm hoping that we can now incrementally improve on what we already have, and not introduce more problems.''.}  \tabularnewline
\midrule
 {Case B: \transcriptEightSCAL: ``When you got 50\% time on this project then you do tend to miss a bit of both'') } \tabularnewline
\midrule
\emph{Inadequately trained development team members} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{2}: ``We did not get any training, we're struggling with it, because it's just a complete different way of thinking for us.  And we have some people naturally fighting against it \ldots{} obviously gonna be more frustrating for the more experienced person who could probably work 2-3 times faster, but it's really about the education, it's what we're trying to achieve.  In theory, hopefully productivity and quality increases as well, two minds on the job, but it's been a struggle.''.}  \tabularnewline
\midrule
 {Case B: \transcriptTwoSCAL: ``\ldots{} myself and [X], even though we did get a bit of training for the [agile team role] stuff, I don't feel like the team had enough training on what our role was.  So, I think our role wasn't done to the best of its ability.'') } \tabularnewline
\midrule
\emph{Ineffective communication} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{2}: ``I've seen problems where people gets too Jira focused, and they stopped talking.  I think there's still a lot of value in us talking to each other, and Jira has sometimes taken that away.  Obviously you've got to find the balance.''.}  \tabularnewline
\midrule
 {Case B: \transcriptSevenSCAL: ``Possibly things would be late if you do not have face-to-face communication we can interpret the things in different way.'') } \tabularnewline
\midrule
\emph{Ineffective project manager}  \tabularnewline
\midrule
\emph{Inexperienced project manager}  \tabularnewline
\midrule
\emph{Inexperienced team members}  \tabularnewline
\midrule
\emph{Lack of an effective project management methodology} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{6}: ``We got a definition of done, in that two weeks period, it has to be coded, documented, and it's got to be QA.  So nothing gets released in those two weeks, if it's not QA.  And also, in the criteria being done, it's as close as possible to 100\% automation\ldots{} it's something we didn't have before.  We used to concentrate on a lot of manual work, now we say to the team, it's just your responsibility as QA to automate.''.}  \tabularnewline
\midrule
 {Case B: \transcriptSevenSCAL: ``\ldots{} it looks like we have waterfall. But, we don't have waterfall, so we are trying to be more Agile.) } \tabularnewline
\midrule
\emph{Lack of commitment to the project among development team members} (observed in Case B) \tabularnewline
\midrule
 {Case B: \Observation: Team members report neutral motivation) } \tabularnewline
\midrule
\emph{Lack of people skills in project leadership}  \tabularnewline
\midrule
\emph{Large number of links to other systems required} (observed in Case B) \tabularnewline
\midrule
 {Case B: \Observation: Changes made by customer teams break features) } \tabularnewline
\midrule
\emph{Negative attitudes by development team} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{2}: ``We didn't make that decision, it was made for us.  But having said that, we still have a degree of team independence, being able to decide how we do things.  Some things are mandatory, sort [of] 50-50, some things are mandated, but we do get to make decisions.''.}  \tabularnewline
\midrule
 {Case B: \Observation: ``We don't trust our {[role in agile team]}'') } \tabularnewline
\midrule
\emph{new: Ineffective collaboration} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{8}: ``The question remains, what's the most effective team size, certainly it's bigger than what we used to have, I’m not sure if it's bigger or smaller than we currently have, but we're doing an experiment with a team of 7, that just starter now,  4 teams, 3 areas about 12-13 engineers, one team is 7 but that's experimental.''.}  \tabularnewline
\midrule
 {Case B: \transcriptOneSCAL: ``We kind of overcommitted the first time. We overcommitted to a lot of stuff, work to be done within the sprint which I think was too much. It is a result of bad or wrong estimation. So, whatever we committed to do in two weeks in reality the job took four weeks.'') } \tabularnewline
\midrule
\emph{new: Ineffective coordination} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{7}: ``when you encounter a support ticket or some other work that's out of line of what your direction and goals are, the impact on your velocity is greater, suddenly you have to do hot fix for production you didn't know about until yesterday, it's gonna take about 2 weeks, effectively half of your team is out for 2 weeks, and your progress is halted.''.}  \tabularnewline
\midrule
 {Case B: \transcriptSixSCAL: ``When we do our coding we have to lock our unit that we are working on.  When we finish the job we commit the code then release the lock,  so someone else can check that unit about what changes. But, sometimes -- well it happens regularly in every week -- that someone forgets to unlock the unit.'') } \tabularnewline
\midrule
\emph{new: Lack of trust} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{8}: ``we struggle with small customers, where they can't afford, or we can't to give them consultant or help, so we really haven't put enough effort in self-service, making it easy to use, a customer can't just sign up and get a trial of the software, they can't just sign up and  pay on the credit card and start using it. It's complete opposite of that, we need many people involved in order to have any customer start using our software.''.}  \tabularnewline
\midrule
 {Case B: \transcriptNineSCAL: ``Yeah, when I say rework its not re-edit.  It's kind of starting from scratch.  So, that is one thing I need to change because I don't think it follows agile to require approval from so many different points.'') } \tabularnewline
\midrule
\emph{One of the largest projects attempted by the organization}  \tabularnewline
\midrule
\emph{Poor project planning} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptOneSCAL: ``You could expect there will be a bottleneck during that time, if it was scheduled properly, job and tasks are completed.  In reality, what happens, all developers finish their tasks around the same time then it's required a lot of responsibilities and time for QA to finish.'') } \tabularnewline
\midrule
\emph{Project affects a large number of user departments or units} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{6}: ``On-premise, you might break one customer.  If you introduce a defect on the cloud, you might break 20 or 50.  Sometime the impact that it has on the cloud is wider.''.}  \tabularnewline
\midrule
\emph{Project involves the use of new technology} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{2}: ``\ldots{} every release, there's one or two items that had to do with other technology, some new tools, some API, some metadata they got, that we need to consume and fit into our model.''.}  \tabularnewline
\midrule
\emph{Project involves use of technology that has not been used in prior projects} (observed in Case B) \tabularnewline
\midrule
 {Case B: \Observation: ``We decided not to do automated testing because this is a legacy product'') } \tabularnewline
\midrule
\emph{Project milestones not clearly defined} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptTwoProgram: ``We tried really hard. It is not in all impossible but we did try and we have succeeded to some extent. And I'd definitely think that if everybody sprints, just the opinion if everybody use sprint team, I think it would be easier to do.'') } \tabularnewline
\midrule
\emph{Project progress not monitored closely enough} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{6}: ``Yes, we still find even, once we get to the final IR, and we've gone to those two weeks getting ready to release to production.''.}  \tabularnewline
\midrule
\emph{Team members lack specialized skills required by the project} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{2}: ``We've all been going into areas we don't have a lot of expertise, like web programming, it wasn't our forte 10 years ago.  And now we definitely have leveraged a lot open source for that kind of thing.''.}  \tabularnewline
\midrule
 {Case B: \transcriptTwoSCAL: ``In this particular project [motivation is] neither low nor high because of the learning curve. And, it's been very difficult to wrap my head around the role itself.  \ldots{} [I]t's been quite demoralizing actually when you don't fully understand your job properly.'') } \tabularnewline
\midrule
\emph{Team members not familiar with the task(s) being automated} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{2}: ``Some things are more straightforward and there's no really architecture.  We certainly look at the risks, like if this going to perform well and we tried to do all that front work.  When you got something like what we're doing right now, rolling out a new dashboard, massive architectural spikes at the start, cause we got to work it out, how to put the data we have, massive amount of data, how to summarize it, and everything have to perform well \ldots{}  bring that kind of stuff to the architecture upfront.''.}  \tabularnewline
\midrule
\textbf{Quadrant 4: Environment} \tabularnewline
\midrule
\emph{Change in organizational management during the project}  \tabularnewline
\midrule
\emph{Corporate politics with negative effect on project}  \tabularnewline
\midrule
\emph{Dependency on outside suppliers} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptTenPortfolio: ``Well, we categorized our epics into different sections and modules based on the multiple different moving parts of the product such as interfaces, contact lens interface, third party company\ldots{}'') } \tabularnewline
\midrule
\emph{Many external suppliers involved in the development project}  \tabularnewline
\midrule
\emph{new: Country-specific regulations} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{8}: ``Yes, the PO were meant to create storyboard for new features, for you to be able to create a storyboard, you've got to be in contact with the Product Management and with sales and service to make sure whatever we produce is suitable for the market and meet customers’ requirements.''.}  \tabularnewline
\midrule
 {Case B: \transcriptTwoPortfolio: ``It is super specific in France, the vertical business is not driven by medical or exam it is mainly driven by retail because it is purely retail and there are many regulations, constraints and rules. So one of the projects we have to manage especially for January [for] example we have new regulations to integrate\ldots{} for the customer.'') } \tabularnewline
\midrule
\emph{new: Delays caused by global distance} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{3}: ``Yes, I think the big eye opener for us is that the operation team is completely independent body based in US, so interacting with them, sometimes we know what the problem is, will be quite easy for us to say just get us the access to machine and I’ll fix it on the spot.But with operation, it doesn't work that way. There's an issue, there's the ticket, and you provide a solution, so it works by raising the ticket.''.}  \tabularnewline
\midrule
 {Case B: \transcriptSixSCAL: ``When we do our coding we have to lock our unit that we are working on.  When we finish the job we commit the code then release the lock,  so someone else can check that unit about what changes. But, sometimes -- well it happens regularly in every week -- that someone forgets to unlock the unit.'') } \tabularnewline
\midrule
\emph{new: Lack of architecture-organization alignment} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{8}: ``Yes, like I said, performance is a constant architectural challenge and we've really struggled with it in the past. Lot of our things in the past were being built without really thinking about it till the end. And we ran into huge problem that way, so we've tried to reverse that, we're tried to push that into the architecture right at the start.''.}  \tabularnewline
\midrule
 {Case B: \transcriptEightSCAL: ``When you got 50\% time on this project then you do tend to miss a bit of both'') } \tabularnewline
\midrule
\emph{new: Lack of face-to-face interaction inhibits knowledge sharing} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{7}: ``For instance, now, we've got an independent test team member who has join our team in inception, but that's not always the case.''.}  \tabularnewline
\midrule
 {Case B: \transcriptEightSCAL: ``When you got 50\% time on this project then you do tend to miss a bit of both'') } \tabularnewline
\midrule
\emph{new: Lack of process alignment} (observed in both cases) \tabularnewline
\midrule
 {Case A: \PA{7}: ``User stories, the way we did it in my old team, usually AO write it on the board, we take a photo and that's your index card.''.}  \tabularnewline
\midrule
 {Case B: \transcriptTwoProgram: ``We tried really hard. It is not in all impossible but we did try and we have succeeded to some extent. And I'd definitely think that if everybody sprints, just the opinion if everybody use sprint team, I think it would be easier to do.'') } \tabularnewline
\midrule
\emph{new: Lack of tool/infrastructure alignment} (observed in Case A) \tabularnewline
\midrule
 {Case A: \PA{6}: ``Yes, we haven't achieved 100\% automation, a lot of people think it's the solution to everything. But you build a component, even though we ask you to provide 100\% automation for cloud and on-prem, there's always a particular failure . So there's component of manual testing and also exploratory testing that we do. Automation has played a bigger role for us, we reduced the release cycle from 6 weeks to 2 weeks, without automation to give us that nightly check ability, it's very difficult, and our product is very complex, just setting up the environment and do manual testing is weeks of effort.''.}  \tabularnewline
\midrule
\emph{new: Unstable country/regional political/economic environment}  \tabularnewline
\midrule
\emph{Organization undergoing restructuring during the project} (observed in Case B) \tabularnewline
\midrule
 {Case B: \transcriptTwoSCAL: ``So, we worked in waterfall fashion in the past and I think this is difficult for people to move from the waterfall way to the Scrum way.'') } \tabularnewline
\midrule
\emph{Resources shifted from the project due to changes in organizational priorities} (observed in Case B) \tabularnewline
\midrule
 {Case B: \Observation: PO responsibilities split between support and PO) } \tabularnewline
\midrule
\emph{Unstable organizational environment}  \tabularnewline


==> verner-wk-mapping-table.tex <==
\midrule
\textbf{Quadrant 1: Customer Mandate} \tabularnewline
\midrule
\emph{Conflict between users} \tabularnewline
\midrule
National, organizational, and cultural differences of participants can cause problems like rework, loss of data, confusions, etc. \tabularnewline
\midrule
\emph{Lack of cooperation from users} \tabularnewline
\midrule
National, organizational, and cultural differences of participants can cause problems like rework, loss of data, confusions, etc. \tabularnewline
\midrule
\emph{Lack of user participation} \tabularnewline
\midrule
National, organizational, and cultural differences of participants can cause problems like rework, loss of data, confusions, etc. \tabularnewline
Lack of collaboration for RE between distributed stakeholders happens due to differences in culture, language distance and processes \tabularnewline
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Requirements information not properly shared with distributed stakeholders affecting their interaction \tabularnewline
\midrule
\emph{Lack or loss of organizational commitment to the project} \tabularnewline
\midrule
Stakeholders are less likely to commit to the project organization and its task when cultural differences and lack of face-to-face interaction makes it difficult to establish a clear project identity \tabularnewline
\midrule
\emph{Users not committed to the project} \tabularnewline
\midrule
Stakeholders are less likely to commit to the project organization and its task when cultural differences and lack of face-to-face interaction makes it difficult to establish a clear project identity \tabularnewline
\midrule
\emph{Users with negative attitudes toward the project} \tabularnewline
\midrule
Lack of informal communication negatively impacts relationship building \tabularnewline
\midrule
\textbf{Quadrant 2: Scope and Requirements} \tabularnewline
\midrule
\emph{Conflicting system requirements} \tabularnewline
\midrule
Lack of a common understanding of requirements leads to problems in system functionality \tabularnewline
Lack of collaboration for RE between distributed stakeholders happens due to differences in culture, language distance and processes \tabularnewline
Requirements information not properly shared with distributed stakeholders affecting their interaction \tabularnewline
\midrule
\emph{Continually changing project scope/objectives} \tabularnewline
\midrule
Risk management including issues related to coordination, problem resolution problem resolution evolving requirements, knowledge sharing, and risk identification \tabularnewline
Task uncertainty represents lack of information needed to develop the software, and it can result in slow change coordination and process and relational conflict \tabularnewline
High organizational complexity, scheduling, task assignment and cost estimation become more problematic in distributed environments as a result of volatile requirements diversity and lack of informal communication \tabularnewline
\midrule
\emph{Continually changing system requirements} \tabularnewline
\midrule
Risk management including issues related to coordination, problem resolution problem resolution evolving requirements, knowledge sharing, and risk identification \tabularnewline
High organizational complexity, scheduling, task assignment and cost estimation become more problematic in distributed environments as a result of volatile requirements diversity and lack of informal communication \tabularnewline
Requirements change management issues can be a problem especially if there are no defined organizational policies \tabularnewline
\midrule
\emph{Difficulty in defining the inputs and outputs of the system} \tabularnewline
\midrule
Lack of effective communication causes problems with knowledge management; participants may lack information about tasks, purpose, and their own contribution overall \tabularnewline
Lack of appropriate information flow throughout the project causes problems with knowledge management \tabularnewline
\midrule
\emph{Ill-defined project goals} \tabularnewline
\midrule
Poor communication bandwidth for agile development causes problems with communication and knowledge management \tabularnewline
Goal distribution can lead to conflicts related to task interpretation, process principles, and problem resolution approaches and can result in site wars and low performance. Goal distribution is more likely in GSD because of faulty transfer of information and a focus on own site performance \tabularnewline
Lack of coordination causes problems such as unclear lines of communication and poor handling of deadlines and milestones \tabularnewline
Problems with tracking and control can lead to unawareness of real project progress \tabularnewline
Task uncertainty represents lack of information needed to develop the software, and it can result in slow change coordination and process and relational conflict \tabularnewline
Lack of common stakeholder goals due to problems of communication and lack of common understanding of requirements \tabularnewline
\midrule
\emph{Incorrect system requirements} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Problems caused because team members do not share equal knowledge of the domain \tabularnewline
Lack of a common understanding of requirements leads to problems in system functionality \tabularnewline
Lack of collaboration for RE between distributed stakeholders happens due to differences in culture, language distance and processes \tabularnewline
\midrule
\emph{System requirements not adequately identified} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
A lack of suitable tools or methodologies available for requirements elicitation may lead to problems in obtaining the real requirements \tabularnewline
Requirements information not properly shared with distributed stakeholders affecting their interaction \tabularnewline
\midrule
\emph{Unclear system requirements} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Cultural diversity between development sites or teams can cause misunderstandings \tabularnewline
Lack of a common understanding of requirements leads to problems in system functionality \tabularnewline
Lack of collaboration for RE between distributed stakeholders happens due to differences in culture, language distance and processes \tabularnewline
Requirements information not properly shared with distributed stakeholders affecting their interaction \tabularnewline
\midrule
\emph{Undefined project success criteria} \tabularnewline
\midrule
Spatial distribution complicates project manager's ability to monitor participants and progress, increases travel budgets, limits face-to-face interaction, and weakens social relations \tabularnewline
Goal distribution can lead to conflicts related to task interpretation, process principles, and problem resolution approaches and can result in site wars and low performance. Goal distribution is more likely in GSD because of faulty transfer of information and a focus on own site performance \tabularnewline
consider adding two other risks: Problems with tracking and control can lead to unawareness of real project progress \tabularnewline
Lack of effective communication causes problems with knowledge management; participants may lack information about tasks, purpose, and their own contribution overall \tabularnewline
\midrule
\emph{Users lack understanding of system capabilities and limitations} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Limited face-to-face meetings caused by geographic distance impact trust, decision quality, creativity, and general management; knowledge creation is limited within organization. This may lead to problems in creating collaboration know-how and domain knowledge \tabularnewline
\midrule
\textbf{Quadrant 3: Execution} \tabularnewline
\midrule
\emph{Development team unfamiliar with selected development tools} \tabularnewline
\midrule
Working with different CM tools can cause slow and unreliable sites, lack of awareness of product changes, and problems with bug fixes between sites \tabularnewline
Working in different SCM environments leads to maintenance requests being handled at several levels in the project \tabularnewline
Selection of inappropriate information and communication technology causes problems such as unreliable networks which may lead to frustration and low efficiency, limit exchange of sensitive information, or even cause production to stop \tabularnewline
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
\midrule
\emph{Frequent conflicts among development team members} \tabularnewline
\midrule
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Cultural bias may lead to erroneous decisions and insecurity about other participants' qualifications and it can have a devastating impact on communication and collaboration efforts. Cultural bias occurs when project participants consider their norms and values as universal and neglect to reflect onto what extent values, norms, and biases are founded in their own cultural background \tabularnewline
Cultural diversity between development sites or teams can cause misunderstandings \tabularnewline
Differences in work culture may render difficulties when sites are different in terms of team behaviour, balancing of collectivism and individualism, perception of authority and hierarchy, planning, punctuality, and organizational culture.  This may lead to decreased conflict handling capabilities and lower efficiency or even paralyse the project \tabularnewline
Not tailoring organizational structures to reduce delays in problem resolution causes difficulties and can result in site wars and reduce project cohesion \tabularnewline
Task uncertainty represents lack of information needed to develop the software, and it can result in slow change coordination and process and relational conflict \tabularnewline
Problems with people management, conflict resolution, and staff turnover are caused by a lack of control \tabularnewline
\midrule
\emph{Frequent turnover within the project team} \tabularnewline
\midrule
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Problems with people management, conflict resolution, and staff turnover are caused by a lack of control \tabularnewline
\midrule
\emph{Immature technology} \tabularnewline
\midrule
Selection of inappropriate information and communication technology causes problems such as unreliable networks which may lead to frustration and low efficiency, limit exchange of sensitive information, or even cause production to stop \tabularnewline
Problems can be caused by the lack of deployment of a configuration management system \tabularnewline
Selection of inappropriate information and communication technology causes problems such as unreliable networks which may lead to frustration and low efficiency, limit exchange of sensitive information, or even cause production to stop \tabularnewline
\midrule
\emph{Inadequate estimation of project budget} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Spatial distribution complicates project manager's ability to monitor participants and progress, increases travel budgets, limits face-to-face interaction, and weakens social relations \tabularnewline
High organizational complexity, scheduling, task assignment and cost estimation become more problematic in distributed environments as a result of volatile requirements diversity and lack of informal communication \tabularnewline
\midrule
\emph{Inadequate estimation of project schedule} \tabularnewline
\midrule
High organizational complexity, scheduling, task assignment and cost estimation become more problematic in distributed environments as a result of volatile requirements diversity and lack of informal communication \tabularnewline
Poor schedule management \tabularnewline
\midrule
\emph{Inadequate estimation of required resources} \tabularnewline
\midrule
Spatial distribution complicates project manager's ability to monitor participants and progress, increases travel budgets, limits face-to-face interaction, and weakens social relations \tabularnewline
High organizational complexity, scheduling, task assignment and cost estimation become more problematic in distributed environments as a result of volatile requirements diversity and lack of informal communication \tabularnewline
\midrule
\emph{Inadequately trained development team members} \tabularnewline
\midrule
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
\midrule
\emph{Ineffective communication} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Lack of synchronous communication in agile development causes problems \tabularnewline
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Poor communication bandwidth for agile development causes problems with communication and knowledge management \tabularnewline
Large teams involved with agile development can cause problems related to communication and coordination \tabularnewline
Working in different SCM environments leads to maintenance requests being handled at several levels in the project \tabularnewline
Language differences between development sites can result in misinterpretations and unconveyed information \tabularnewline
Cultural bias may lead to erroneous decisions and insecurity about other participants' qualifications and it can have a devastating impact on communication and collaboration efforts. Cultural bias occurs when project participants consider their norms and values as universal and neglect to reflect onto what extent values, norms, and biases are founded in their own cultural background \tabularnewline
Cultural diversity between development sites or teams can cause misunderstandings \tabularnewline
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
Limited possibility for informal communication due to dispersion of sites (i.e., lack of spontaneous communication) causes problems with social integration of teams \tabularnewline
Lack of effective communication causes problems with knowledge management; participants may lack information about tasks, purpose, and their own contribution overall \tabularnewline
Inability to communicate in real time) causes collaboration problems \tabularnewline
It may be difficult to establish effective coordination mechanisms in projects and overcome challenges such as little face-to-face interaction, problematic task coupling, different time zones, local holidays, weak social networks, and unclear communication lines \tabularnewline
Problems caused by poor collaboration and communication infrastructure \tabularnewline
Use of interaction media may cause problems such as jumbled messages; mix-ups and loss of contextual information. Such problems, may lead to confusion and misunderstandings among participants and lower morale \tabularnewline
Selection of inappropriate information and communication technology causes problems such as unreliable networks which may lead to frustration and low efficiency, limit exchange of sensitive information, or even cause production to stop \tabularnewline
Without communication protocols effective communication can be impeded \tabularnewline
Language and cultural barriers cause problems between client and vendor \tabularnewline
A communication gap between client and vendor may lead to misunderstandings \tabularnewline
Lack of informal communication negatively impacts relationship building \tabularnewline
Stakeholders located in different time zones can lead to problems in communicating \tabularnewline
\midrule
\emph{Ineffective project manager} \tabularnewline
\midrule
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
Poor quality management \tabularnewline
Choosing a vendor with a lack of project management skills can result in difficulties \tabularnewline
\midrule
\emph{Inexperienced project manager} \tabularnewline
\midrule
Choosing a vendor with a lack of project management skills can result in difficulties \tabularnewline
\midrule
\emph{Inexperienced team members} \tabularnewline
\midrule
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
\midrule
\emph{Lack of an effective project management methodology} \tabularnewline
\midrule
Temporal and physical distribution increases complexity of planning and coordination activities, makes multisite virtual meetings hard to plan, causes unproductive waits, delays feedback, and complicates simple things \tabularnewline
Poor quality management \tabularnewline
Risk management including issues related to coordination, problem resolution problem resolution evolving requirements, knowledge sharing, and risk identification \tabularnewline
Lack of coordination causes problems such as unclear lines of communication and poor handling of deadlines and milestones \tabularnewline
Problems with tracking and control can lead to unawareness of real project progress \tabularnewline
Poor control results in lack of effective scope and change management \tabularnewline
Disorganized task allocation leads to some work being done twice and other work omitted \tabularnewline
Lack of control results in no transparency or visibility of project status to all sites involved in project \tabularnewline
Poor schedule management \tabularnewline
Choosing a vendor with a lack of project management skills can result in difficulties \tabularnewline
A vendor with poor contract management can cause problems for the client such as lack of integrity in obligations, commitments and behaviou \tabularnewline
Problems caused by asymmetry in processes, policies and standards \tabularnewline
\midrule
\emph{Lack of commitment to the project among development team members} \tabularnewline
\midrule
Stakeholders are less likely to commit to the project organization and its task when cultural differences and lack of face-to-face interaction makes it difficult to establish a clear project identity \tabularnewline
\midrule
\emph{Lack of people skills in project leadership} \tabularnewline
\midrule
Problems with people management, conflict resolution, and staff, turnover are caused by a lack of control \tabularnewline
\midrule
\emph{Negative attitudes by development team} \tabularnewline
\midrule
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Cultural bias may lead to erroneous decisions and insecurity about other participants qualifications and it can have a devastating impact on communication and collaboration efforts. Cultural bias occurs when project participants consider their norms and values as universal and neglect to reflect onto what extent values, norms, and biases are founded in their own cultural background \tabularnewline
\midrule
\emph{new: Lack of architecture-organization alignment} \tabularnewline
\midrule
Lack of well-defined modules causes problems with progressive integration \tabularnewline
High task coupling between task segments increases the need for inter-site communication, coordination, and integration, and it can lead to lower level of performance as well as increase the number of failures \tabularnewline
\midrule
\emph{new: Lack of trust} \tabularnewline
\midrule
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Mutual trust is important but hard to obtain and lack of trust causes problems. This can be due to lack of face-to-face interaction, cultural differences, and weak social relations \tabularnewline
Fear about the future of jobs and roles, erodes trust \tabularnewline
Limited face-to-face meetings caused by geographic distance impact trust, decision quality, creativity, and general management; knowledge creation is limited within organization. This may lead to problems in creating collaboration know-how and domain knowledge \tabularnewline
Trust among stakeholders necessary to achieve innovation, flexibility, cooperation, and efficiency in distributed environment. Since often a short life span, important to achieve mutual trust rapidly, but if trust is misplaced, entire organization may suffer \tabularnewline
A vendor with poor relationship management can result in problems such as lack of trust \tabularnewline
\midrule
\emph{Poor project planning} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Lack of project planning causes problems \tabularnewline
Poor identification of roles and responsibilities \tabularnewline
Lack of detailed planning causes problems with task allocation \tabularnewline
\midrule
\emph{Project affects a large number of user departments or units} \tabularnewline
\midrule
Organizational challenges caused by GSD beyond distance and cultural differences, e.g., if the client organization has a large number of stakeholders, and /or the vendor organization has a number of sites \tabularnewline
Large teams involved with agile development can cause problems related to communication and coordination \tabularnewline
\midrule
\emph{Project involves use of technology that has not been used in prior projects} \tabularnewline
\midrule
Working with different CM tools can cause slow and unreliable sites, lack of awareness of product changes, and problems with bug fixes between sites \tabularnewline
Working in different SCM environments leads to maintenance requests being handled at several levels in the project \tabularnewline
Choosing a vendor with a lack of technical capability can result in problems \tabularnewline
\midrule
\emph{Project milestones not clearly defined} \tabularnewline
\midrule
Lack of coordination causes problems such as unclear lines of communication and poor handling of deadlines and milestones \tabularnewline
\midrule
\emph{Project progress not monitored closely enough} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Lack of coordination causes problems such as unclear lines of communication and poor handling of deadlines and milestones \tabularnewline
Problems with tracking and control can lead to unawareness of real project progress \tabularnewline
Lack of control results in no transparency or visibility of project status to all sites involved in project \tabularnewline
Poor schedule management \tabularnewline
Spatial distribution complicates project manager's ability to monitor participants and progress, increases travel budgets, limits face-to-face interaction, and weakens social relations \tabularnewline
\midrule
\emph{Team members lack specialized skills required by the project} \tabularnewline
\midrule
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
Difficulties caused by different knowledge levels or knowledge transfer problems \tabularnewline
Choosing a vendor with a lack of technical capability can result in problems \tabularnewline
\midrule
\emph{Team members not familiar with the task(s) being automated} \tabularnewline
\midrule
Difficulties caused by different knowledge levels or knowledge transfer problems \tabularnewline
Problems caused because team members do not share equal knowledge of the domain \tabularnewline
Lack of appropriate information flow throughout the project causes problems with knowledge management \tabularnewline
Task uncertainty represents lack of information needed to develop the software, and it can result in slow change coordination and process and relational conflict \tabularnewline
\midrule
\textbf{Quadrant 4: Environment} \tabularnewline
\midrule
\emph{Dependency on outside suppliers} \tabularnewline
\midrule
Vendor's strategic inflexibility can result in major disagreements \tabularnewline
Vendor's poor infrastructure such as infrastructure incompatibility between sites causes problems; selection of appropriate information and communication technology is crucial for project success \tabularnewline
Lack of protection for intellectual property rights in the vendor country \tabularnewline
Problems because of differences in legal systems such as jurisdiction, patents, and International laws \tabularnewline
Vendor country instability such as political instability, corruption, peace problems, terrorism threats and uncertainty relating to trade and investment can cause project difficulties \tabularnewline
Vendor's behaves opportunistically \tabularnewline
Vendor has previous delays in delivery so may be unreliable \tabularnewline
Vendor incompatibility with client causes problems \tabularnewline
Choosing a vendor with a lack of project management skills can result in difficulties \tabularnewline
Choosing a vendor with a lack of technical capability can result in problems \tabularnewline
A vendor with poor contract management can cause problems for the client such as lack of integrity in obligations, commitments and behaviou \tabularnewline
A vendor with poor quality of service and systems/processes can result in problems \tabularnewline
Hidden vendor costs can be expensive \tabularnewline
Choosing a vendor with a lack of control over a project can result in problems such as cost and schedule overruns \tabularnewline
\midrule
\emph{new: Country-specific regulations} \tabularnewline
\midrule
Lack of protection for intellectual property rights in the vendor country \tabularnewline
Problems because of differences in legal systems such as jurisdiction, patents, and International laws \tabularnewline
\midrule
\emph{new: Delays caused by global distance} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Configuration management problems cause dependency, delay and increased time is required to complete maintenance requests \tabularnewline
Temporal and physical distribution increases complexity of planning and coordination activities, makes multisite virtual meetings hard to plan, causes unproductive waits, delays feedback, and complicates simple things \tabularnewline
Inability to communicate in real time) causes collaboration problems; \tabularnewline
Stakeholders located in different time zones can lead to problems in communicating \tabularnewline
Not tailoring organizational structures to reduce delays in problem resolution causes difficulties and can result in site wars and reduce project cohesion \tabularnewline
Choosing a vendor with a lack of control over a project can result in problems such as cost and schedule overruns; and Poor schedule management \tabularnewline
\midrule
\emph{new: Ineffective collaboration} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Lack of tool support for agile development causes problems with agile practices \tabularnewline
Cultural bias may lead to erroneous decisions and insecurity about other participants' qualifications and it can have a devastating impact on communication and collaboration efforts. Cultural bias occurs when project participants consider their norms and values as universal and neglect to reflect onto what extent values, norms, and biases are founded in their own cultural background \tabularnewline
Lack of training in communication and collaboration tools causes problems with communication \tabularnewline
Limited possibility for informal communication due to dispersion of sites (i.e., lack of spontaneous communication) causes problems with social integration of teams \tabularnewline
Inability to communicate in real time) causes collaboration problems \tabularnewline
Problems caused by poor collaboration and communication infrastructure \tabularnewline
Selection of inappropriate information and communication technology causes problems such as unreliable networks which may lead to frustration and low efficiency, limit exchange of sensitive information, or even cause production to stop \tabularnewline
Language and cultural barriers cause problems between client and vendor \tabularnewline
Lack of collaboration for RE between distributed stakeholders happens due to differences in culture, language distance and processes \tabularnewline
\midrule
\emph{new: Ineffective coordination} \tabularnewline
\midrule
Problems caused by asymmetry in processes, policies and standards \tabularnewline
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Lack of synchronous communication in agile development causes problems \tabularnewline
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Poor communication bandwidth for agile development causes problems with communication and knowledge management \tabularnewline
Lack of tool support for agile development causes problems with agile practices \tabularnewline
Large teams involved with agile development can cause problems related to communication and coordination \tabularnewline
High task coupling between task segments increases the need for inter-site communication, coordination, and integration, and it can lead to lower level of performance as well as increase the number of failures \tabularnewline
Temporal and physical distribution increases complexity of planning and coordination activities, makes multisite virtual meetings hard to plan, causes unproductive waits, delays feedback, and complicates simple things \tabularnewline
It may be difficult to establish effective coordination mechanisms in projects and overcome challenges such as little face-to-face interaction, problematic task coupling, different time zones, local holidays, weak social networks, and unclear communication lines \tabularnewline
Lack of coordination causes problems such as unclear lines of communication and poor handling of deadlines and milestones \tabularnewline
Coordination in multisite development becomes more difficult in terms of articulation of work as problems from communication lack of group awareness and complexity of the organization appear and influence the way the work must be structured \tabularnewline
\midrule
\emph{new: Lack of face-to-face interaction inhibits knowledge sharing} \tabularnewline
\midrule
Application of agile practices causes problems in distributed development because of the degree of interaction between stakeholders and number of face-to-face meetings needed \tabularnewline
Collaboration difficulties caused by geographic distance in agile development may cause misunderstandings and conflicts \tabularnewline
Poor communication bandwidth for agile development causes problems with communication and knowledge management \tabularnewline
Project participants have limited understanding of other project participants' competencies \tabularnewline
Lack of team cohesiveness causes problems as some members feel isolated from other team members; participants have limited understanding of other project participants' competencies \tabularnewline
Limited face-to-face meetings caused by geographic distance impact trust, decision quality, creativity, and general management; knowledge creation is limited within organization. This may lead to problems in creating collaboration know-how and domain knowledge \tabularnewline
Temporal and physical distribution increases complexity of planning and coordination activities, makes multisite virtual meetings hard to plan, causes unproductive waits, delays feedback, and complicates simple things \tabularnewline
Coordination in multisite development becomes more difficult in terms of articulation of work as problems from communication lack of group awareness and complexity of the organization appear and influence the way the work must be structured \tabularnewline
Spatial distribution complicates project manager's ability to monitor participants and progress, increases travel budgets, limits face-to-face interaction, and weakens social relations \tabularnewline
\midrule
\emph{new: Lack of process alignment} \tabularnewline
\midrule
Problems caused by asymmetry in processes, policies and standards \tabularnewline
No process alignment, in terms of traditions, development methods, and emphasis on user involvement, will often differentiate between sites, possibly resulting in incompatibility and conflicts \tabularnewline
National, organizational, and cultural differences of participants can cause problems like rework, loss of data, confusions, etc. \tabularnewline
\midrule
\emph{new: Lack of tool/infrastructure alignment} \tabularnewline
\midrule
Tool compatibility may prove a problem; sites are likely to prefer different programming languages, support tools, operating systems, and development tools \tabularnewline
Vendor's poor infrastructure such as infrastructure incompatibility between sites causes problems; selection of appropriate information and communication technology is crucial for project success \tabularnewline
\midrule
\emph{new: Unstable country/regional political/economic environment} \tabularnewline
\midrule
Vendor country instability such as political instability, corruption, peace problems, terrorism threats and uncertainty relating to trade and investment can cause project difficulties \tabularnewline

